DeFiRanger: Detecting Price Manipulation Attacks on DeFi Applications

The rapid growth of Decentralized Finance (DeFi) boosts the Ethereum ecosystem. At the same time, attacks towards DeFi applications (apps) are increasing. However, to the best of our knowledge, existing smart contract vulnerability detection tools cannot be directly used to detect DeFi attacks. That's because they lack the capability to recover and understand high-level DeFi semantics, e.g., a user trades a token pair X and Y in a Decentralized EXchange (DEX). In this work, we focus on the detection of two types of new attacks on DeFi apps, including direct and indirect price manipulation attacks. The former one means that an attacker directly manipulates the token price in DEX by performing an unwanted trade in the same DEX by attacking the vulnerable DeFi app. The latter one means that an attacker indirectly manipulates the token price of the vulnerable DeFi app (e.g., a lending app). To this end, we propose a platform-independent way to recover high-level DeFi semantics by first constructing the cash flow tree from raw Ethereum transactions and then lifting the low-level semantics to high-level ones, including token trade, liquidity mining, and liquidity cancel. Finally, we detect price manipulation attacks using the patterns expressed with the recovered DeFi semantics. We have implemented a prototype named \tool{} and applied it to more than 350 million transactions. It successfully detected 432 real-world attacks in the wild. We confirm that they belong to four known security incidents and five zero-day ones. We reported our findings. Two CVEs have been assigned. We further performed an attack analysis to reveal the root cause of the vulnerability, the attack footprint, and the impact of the attack. Our work urges the need to secure the DeFi ecosystem.

==> JavaScript-highlighting.tex <==
\usepackage{listings, xcolor}

\definecolor{verylightgray}{rgb}{.97,.97,.97}

\lstdefinelanguage{JavaScript}%
  {morekeywords={typeof,new,true,false,catch,function,return,null,catch,switch,var,if,in,while,do,else,case,break},%
  morecomment=[l]//,%
  morecomment=[s]{/*}{*/},%
  morestring=[b]",%
  morestring=[b]',%
  }[keywords,comments,strings]%
  

==> figures/artem_arbitrage.tex <==
\begin{figure}[t]
    \includegraphics[width=0.48\textwidth]{pdfs/artem_arbitrage.pdf}
    \caption{Artem~\cite{Artem} price feeding frequency. Three lines refer to the price trend in three DEXs' ETH-related 
    pools. A dot in a line indicate that Artem is fed the price of line-related asset, USDC, SUSHI, or UNI, at 
    that time.}
	\label{fig:artem}
\end{figure}


==> figures/change_trend.tex <==
\begin{figure}[t]
	\center
	\includegraphics[width=0.48\textwidth]{pdfs/trend.pdf}
    \caption{Ethereum ecosystem changes. \\
    16-10: The DDoS attack~\cite{DDoS} created abnormal high number of useless contracts and internal transactions;\\
    18-11: The start date of the most popular DEX: Uniswap.}
	\label{fig:change_trend}
\end{figure}



==> figures/curve_swap.tex <==
\begin{figure}[t]
	\center
	\hspace*{0.02\textwidth}\includegraphics[width=0.48\textwidth]{pdfs/curve_swap_v2.pdf}
	\caption{Curve~\cite{curve} trade.}
	\label{fig:curve_swap}
\end{figure}



==> formulas/DRC_slippage.tex <==
\begin{equation}
    \label{formula:DRC_slippage}
        \begin{aligned}
            & CurrentUP_{DRC}: \textit{the current unit price of DRC in DEX}  \\
            & LastUP_{DRC}: \textit{the last updated unit price of DRC in DEX} \\ 
            & Slippage = \frac{CurrentUP_{DRC} - LastUP_{DRC}}{LastUP_{DRC}} \\
            & Slippage <= 0.3 \\
        \end{aligned}
\end{equation}


==> formulas/LRC_slippage.tex <==
\begin{equation}
    \label{formula:LRC_slippage}
        \begin{aligned}
            & F(x): \textit{the amount of LRC that x source asset will swap for} \\
            & Slippage = \frac{F(x) * 2- F(2x)}{F(x)} \\
            & Slippage <= 100 \\
        \end{aligned}
\end{equation}


==> formulas/cft_definition.tex <==
\begin{equation}
    \label{formula:definition}
    \begin{aligned}
    & CFT & = & & & (root, F)  \\
    & F & = & & & \left\{
        \begin{aligned}
        & \emptyset \\
        & \{<T_i>| i = 1, 2, 3, ..., n, n>=1\} \\
        \end{aligned}
        \right. \\
    & T_i & = & & & (root_i, F_i) \\
    \end{aligned}
\end{equation}
    

==> formulas/its_trigger.tex <==
\begin{equation}
    \label{formula:its_trigger}
    \left\{
    \begin{aligned}
        & \internal{}_j.\depth{} > \internal{}_1.\depth{}, & 1<j<i \\
        & \internal{}_i.\depth{} <= \internal{}_1.\depth{} \\
        & \internal{}_j.\depth{} > \internal{}_i.\depth{}, & i<j<=n \\
    \end{aligned}
    \right.
\end{equation}


==> tables/artem_arbitrage.tex <==
\begin{table}[t]
	\caption{ The process of Artem arbitrage. }
	\label{tab:artem}
	\centering
    \begin{tabular}{lll}
        \textbf{Action} & \textbf{Change} & \multicolumn{1}{l}{\begin{tabular}[l]{@{}l@{}}\textbf{Arbitrager}\\\textbf{Balance}\end{tabular}} \\
        \toprule
        $1$. Flash loan          & $+21000$ Ether    & $+21000$ Ether  \\
        \hline
        $2$. Swap for SUSHI              & $-167$ Ether    & $+20.8K$ Ether \\
        in a on-chain exchange      & $+74K$ SUSHI  & $+74K$ SUSHI  \\    
        \hline
        $3$. Borrow from Artem           & $-74K$ SUSHI  & $+20832$ Ether\\
                                    & $+63K$ USDC   & $+63K$ USDC \\
                                    & $+51K$ USDT   & $+51K$ USDT \\
                                    & $+599$ UNI    & $+599$ UNI \\
        \hline
        $4$. Swap for Ether                & $-63K$ USDC   & $+21024$ Ether\\
        in on-chain exchanges        & $-51K$ USDT   & \\
                                    & $-599$ UNI    & \\ 
                                    & $+193$ Ether    & \\
        \hline
        $5$. Repay flash loan    & $-21000$       & \textbf{+24 Ether}$^{\rm a}$ \\
        \bottomrule
     \end{tabular}

    \begin{tablenotes}
        \item $\rm a$: $24$ Ether was worth around $14.6K$ USD on the day of the Artem attack.
    \end{tablenotes}

% \vspace{-10pt}
\end{table}


==> tables/attack_division.tex <==
\begin{table}[t]
	\caption{ Attack division }
	\label{tab:attack_division}
	\centering
    \begin{tabular}{lccc}
        \toprule
        \textbf{Attack} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}c@{}}\textbf{\# Attack}\\\textbf{operator}\end{tabular}} 
        & \multicolumn{1}{l}{\begin{tabular}[c]{@{}c@{}}\textbf{\# Malicious}\\\textbf{contract}\end{tabular}} 
        & \multicolumn{1}{l}{\begin{tabular}[c]{@{}c@{}}\textbf{\# Money}\\\textbf{washer}\end{tabular}} \\
        \hline
        Harvest Hack        & $1$ & $1$ & $1$ \\
        Plouto Hack         & $1$ & $1$ & $1$ \\
        Cheese Bank Incident& $1$ & $1$ & $1$ \\
        Value DeFi Incident & $1$ & $1$ & $1$ \\
        WarpFinance Incident& $1$ & $1$ & $1$ \\
        
        \bottomrule
 	\end{tabular}
% \vspace{-10pt}
\end{table}


==> tables/dex_amm_pltf.tex <==
\begin{table*}[t]
	\caption{Difference between classic AMM DEX}
	\label{tbl:AMM_DEX}
	\centering
	\begin{tabular}{|l|c|c|c|}
		\hline        		
		{\bf Providers} &  {\bf Uniswap~\cite{Uniswap-V1,Uniswap-V2}} &  {\bf Balancer~\cite{balancer}} & {\bf Curve.fi~\cite{curve}}   \\
		\hline
		{\it Price Mechanism}      & Constant Product   & ?? & Combined Curves* \\
		\hline
		{\it Distinct Tokens in the Pool} & =2 & 2-8 & >=2 \\
		\hline
		{\it Expected Weight of each Token} & Equivalent & Self-defined & Equivalent\\
		\hline
		{\it Operation Fee}      & Low(0.3\%) & High(0.0001\%-10\%) & Very low(0.04\%) \\
		\hline
 	\end{tabular}

 \begin{tablenotes}
      %\small
      \item * The price calculation formula is not fully transparent to the public\cite{}.
\end{tablenotes}
 \vspace{-10pt}
\end{table*}

==> tables/direct_pricemani_attacks.tex <==
\begin{table*}[t]
	\centering
	\caption{The details of indirect \pricemani{} attacks.}
	% \small
	\resizebox{1.0\textwidth}{!}{
	\begin{tabular}{llllll}
    \toprule
    \textbf{Incident} & \textbf{Price Manipulation 1} & \textbf{Price Manipulation 2} & \textbf{Cost Withdrawal + Profit} \\
    \midrule
    \multirow{6}{1in}{~}& Attacker                  & Attacker invoke \textit{sellTokenForLRC} of LRC   & \\ 
                        & Sell $4.228K$ ETH         & Sell $10$ ETH                                     & Attacker \\
    LRC Incident        & For $4.344K$ LRC          & For $0.0069$ LRC                                  & Sell $4.344K$ LRC \\
                        & In Uniswap V1 ETH-LRC pool& In Uniswap V1 ETH-LRC pool                        & For $4.238K$ ETH \\
                        & To manipulate             & To manipulate                                     & In Uniswap V1 ETH-LRC pool \\
                        & Uniswap V1 ETH-LRC pool   & Uniswap V1 ETH-LRC pool                           & \\
    \hdashline
    Attacker Balance    & $-4.228K$ ETH             & -                         & $+10ETH$  \\
                        & $+4.344K$ LRC             & -                         &           \\
    \midrule
    \multirow{6}{1in}{~}& Attacker                      & Attacker invoke \textit{drain} of Dracula & \\
                        & Sell $124.84$ ETH             & To drain out yields of $23$ pools         & Attacker \\
    DRC Incident        & For $232K$ DRC                & For $7.814K$ DRC                          & Sell $232K$ DRC \\
                        & In Uniswap V2 DRC-ETH pool    & In Uniswap V2 DRC-ETH pool                & For $125.18$ ETH \\
                        & To manipulate                 & To manipulate                             & In Uniswap V2 DRC-ETH pool \\
                        & Uniswap V2 DRC-ETH pool       & Uniswap V2 DRC- ETH pool                  & \\
    \hdashline
    Attacker Balance    & $-124.84K$ ETH                & -                                         & $+0.34$ ETH \\
                        & $+232K$ DRC                   & -                                         &           \\
    \midrule
    \multirow{6}{1in}{~}& Attacker                      & Attacker invoke \textit{breed} of SEAL   & \\ 
                        & Sell $1.084K$ SEAL            & Mint $27$ SEAL                            & Attacker \\
    SEAL Incident       & For $2.787K$ SNX              & To Uniswap V2 SEAL-SNX pool               & Sell $2.787K$ LRC \\
                        & In Uniswap V2 SEAL-SNX pool   & To manipulate                             & For $1.1K$ SEAL \\
                        & To manipulate                 & Uniswap V2 SEAL-SNX pool                  & In Uniswap V2 SEAL-SNX pool \\
                        & Uniswap V2 SEAL-SNX pool      &                                           & \\
    \hdashline
    Attacker Balance    & $-1.084K$ SEAL                & -                                         & $+16$ SEAL \\
                        & $+2.787K$ SNX                 & -                                         &           \\
    \midrule
    \multirow{6}{1in}{~}& Attacker                      & Attacker invoke \textit{closeAuction} of Metronome & \\
                        & Sell $80.79$ ETH              & Send $22.5$ ETH                                    & Attacker \\
    MET incident        & For $37.86K$ MET              & To Metronome AMM pool                              & Sell $37.86K$ MET \\
                        & To manipulate                 & To manipulate                                      & For $80.94$ ETH \\
                        & Metronome AMM pool            & Metronome AMM pool                                 & Metronome AMM pool \\
    \hdashline
    Attacker Balance    & $-80.79$ ETH                  & -                                                  & $+0.15$ ETH \\
                        & $+37.86K$ MET                 & -                                                  & \\
    \bottomrule
\end{tabular}
}


\label{tab:direct_pricemani_attacks}
% \vspace{-0.2in}
\end{table*}


==> tables/indirect_pricemani_attacks.tex <==
\begin{table*}[t]
	\centering
	\caption{The details of indirect \pricemani{} attacks.}
	\small
	\resizebox{1.0\textwidth}{!}{
	\begin{tabular}{llllll}
    \toprule
    \textbf{Incident} & \textbf{Preparation} & \textbf{Price Manipulation} & \textbf{Profit} & \textbf{Cost Withdrawal} & \textbf{Aftercare} \\
    \midrule
    \multirow{5}{1in}{~}                & & Sell $17.89M$ USDT          &                       & Sell $17.91M$ USDC        &                           \\
                                        & & For $17.89M$ USDC           & Deposit $60.2M$ USDC  & For $17.91M$ USDT         &  Burn $69.7M$ fUSDC       \\
    Harvest Hack~\cite{Harvest-hack}    & - & In Curve y pool             & To mint $69.7M$ fUSDC    & In Curve y pool        &  To redeem $60.6M$ USDC   \\
                                        & & To manipulate yCrv's price  & In fUSDC Vault      & To recover yCrv's price   &  In fUSDC Vault         \\
                                        & & In Harvest's fUSDC Vault    &                       & In fUSDC Vault            &                           \\
    \hdashline
                                        & & $-17.89M$ USDT              & $-17.89M$ USDT        & $0.02M$ USDT              & $0.02M$ USDT \\
    Attacker Balance                    & & $+17.89M$ USDC              & $-42.31M$ USDC        & $-60.22M$ USDC            & $0.38M$ USDC \\
                                        & &                             & $+69.7M$ fUSDC        & $+69.7M$ fUSDC            & \\
    \midrule
    \multirow{5}{1in}{~}                & & Sell $9M$ USDC              &                       & Sell $8.21M$ USDT         &                           \\
                                        & & For $8.21M$ USDT            & Deposit $2M$ USDT     & For $8.99M$ USDC          &  Burn $4.22M$ pUSDT       \\
    Plouto Hack~\cite{Plouto-hack}    & - & In Swerve sUSD v2 pool      & To mint $4.22M$ pUSDT & In Swerve sUSD v2 pool    &  To redeem $2.2M$ USDT   \\
                                        & & To manipulate swUSD's price & In pUSDT Vault        & To recover swUSD's price  &  In pUSDT Vault         \\
                                        & & In Plouto's pUSDT Vault     &                       & In pUSDT Vault            &                           \\
    \hdashline
                                        & & $-9M$ USDC                  & $-9M$ USDC            & $-0.01M$ USDC             & $-0.01M$ USDC \\
    Attacker Balance                    & & $+8.21M$ USDT               & $+6.21M$ USDT         & $-2M$ USDT                & $+0.2M$ USDC \\
                                        & &                             & $+4.22M$ pUSDT        & $+4.22M$ pUSDT            & \\
    \midrule
    \multirow{5}{1in}{~}                                &                           & Sell $20K$ ETH                & Deposit $2.8K$ UNI\_V2        &                   &  \\
                                                        & Deposit $128$ ETH         & For $288K$ CHEESE             & As collateral to borrow out   & Sell $288K$ CHEESE&  \\
    Cheese Bank Incident~\cite{Cheese-bank-incident}    & To mint $2.8K$ UNI\_V2    & In Uniswap V2                 & $2.07M$ USDC, $1.23M$ USDT    & For $19.98K$ ETH  &  - \\
                                                        & In Uniswap V2             & To manipulate UNI\_V2's price & $87.6K$ Dai                   & In Uniswap V2     &  \\
                                                        &                           & In Cheese Bank                & In Cheese Bank                &                   &  \\
    \hdashline
                                                        & $-128$ ETH                & $-19.87K$ ETH                 & $-19.87K$ ETH                 & $10$ ETH $^{\rm a}$ &  \\
                                                        & $+2.8K$ UNI\_V2           & $+2.8K$ UNI\_V2               & $+288K$ CHEESE                & $+2.07M$ USDC &  \\
    Attacker Balance                                    &                           & $+288K$ CHEESE                & $+2.07M$ USDC                 & $+1.23M$ USDT &  \\
                                                        &                           &                               & $+1.23M$ USDT                 & $+87.6K$ Dai  &  \\
                                                        &                           &                               & $+87.6K$ Dai                  &  & \\
    \midrule
    \multirow{5}{1in}{~}                                &                           & Sell $91M $ Dai, $31M$ USDT   &                               & Sell $107.62M$ USDC               &  \\
                                                        & Deposit $25M$ Dai         & For $107.62M$ USDC            & Burn $24.9M$ mvUSD            & For $30.94M$ USDT, $90.93M$ Dai   &  Burn $33.09M$ 3Crv \\
    Value DeFi Incident~\cite{Value-incident}           & To mint $24.9M$ mvUSD     & In Curve $3$ pool             & To redeem $33.09M$ 3Crv       & In Curve $3$ pool                 &  To redeem $33.11M$ Dai \\
                                                        & In Value Vaults           & To manipulate 3Crv's price    & In Value Vaults               & To recover 3Crv's price           &  In Curve $3$ pool\\
                                                        &                           & In Value Vaults               &                               & In Value Vaults                   & \\                
    \hdashline
                                                        & $-25M$ Dai                & $-116M$ Dai                   & $-116M$ Dai                    & $-25.07M$ Dai & $8.04M$ Dai \\
    Attacker Balance                                    & $+24.9M$ mvUSD            & $+24.9M$ mvUSD                & $-31M$ USDT                    & $-0.06M$ USDT & $-0.06M$ USDT \\
                                                        &                           & $-31M$ USDT                   & $+107.62M$ USDC                 & $+33.09M$ 3Crv & \\
                                                        &                           & $+107.62M$ USDC                & $+33.09M$ 3Crv                  &               & \\
    \midrule
    \multirow{5}{1in}{~}                                &                               & Sell $341.2K$ ETH             & Deposit $94.35K$ UNI\_V2      &                   &  \\
                                                        & Deposit $2.9M$ Dai, $76K$ ETH & For $47.6M$ Dai               & As collateral to borrow out   & Sell $48.6M$ Dai  &  \\
    WarpFinance Incident~\cite{WarpFinance-incident}    & To mint $94.35K$ UNI\_V2      & In Uniswap V2                 & $3.86M$ Dai                   & For $342.3K$ ETH  &  - \\
                                                        & In Uniswap V2                 & To manipulate UNI\_V2's price & $3.9M$ USDC                   & In Uniswap V2     &  \\
                                                        &                               & In WarpFinance                & In WarpFinance                &                   & \\
    \hdashline
                                                        & $-2.9M$ Dai                   & $+44.7M$ Dai                  & $+48.56M$ Dai                 & $-0.04M$ Dai  & \\
    Attacker Balance                                    & $-76K$ ETH                    & $-417.2K$ ETH                 & $-417.2K$ ETH                 & $-74.9K$ ETH $^{\rm b}$  & \\
                                                        & $+94.35K$ UNI\_V2             & $+94.35K$ UNI\_V2             & $+3.9M$ USDC                  & $+3.9M$ USDC  & \\
    \bottomrule
\end{tabular}}

% \begin{tablenotes}
%     \item $\rm a$: $10$ ETH was worth around $4.2K$ USD on the day of the Cheese Bank Incident.
%     \item $\rm b$: $74.9$ ETH was worth around $47.64K$ USD on the day of the WarpFinance Incident.
%     \item USDC, USDT, DAI all are stable-coins of USD.
% \end{tablenotes}

\label{tab:indirect_pricemani_attacks}
% \vspace{-0.2in}
\end{table*}

